The NANOGrav 12.5-year Data Set: Search For An Isotropic Stochastic Gravitational-Wave Background

We search for an isotropic stochastic gravitational-wave background (GWB) in the $12.5$-year pulsar timing data set collected by the North American Nanohertz Observatory for Gravitational Waves. Our analysis finds strong evidence of a stochastic process, modeled as a power-law, with common amplitude and spectral slope across pulsars. The Bayesian posterior of the amplitude for an $f^{-2/3}$ power-law spectrum, expressed as the characteristic GW strain, has median $1.92 \times 10^{-15}$ and $5\%$--$95\%$ quantiles of $1.37$--$2.67 \times 10^{-15}$ at a reference frequency of $f_\mathrm{yr} = 1 ~\mathrm{yr}^{-1}$. The Bayes factor in favor of the common-spectrum process versus independent red-noise processes in each pulsar exceeds $10,000$. However, we find no statistically significant evidence that this process has quadrupolar spatial correlations, which we would consider necessary to claim a GWB detection consistent with general relativity. We find that the process has neither monopolar nor dipolar correlations, which may arise from, for example, reference clock or solar system ephemeris systematics, respectively. The amplitude posterior has significant support above previously reported upper limits; we explain this in terms of the Bayesian priors assumed for intrinsic pulsar red noise. We examine potential implications for the supermassive black hole binary population under the hypothesis that the signal is indeed astrophysical in nature.

==> table_commonprocess_bfs.tex <==
% !TEX root = nanograv_12p5yr_gwb.tex

\begin{table*}
  \begin{center}
  \caption{Uncorrelated common process posteriors for the NANOGrav 12.5-year data set. We report the mean value, along with the standard deviation, of the amplitude for a power-law spectrum with $\gamma = 13/3$, as well as the Bayes factors for a model comparison between an uncorrelated common process and no common process (pulsar noise only). The Bayes factors were computed with the product-space method discussed in Sec.\ \ref{sec:data_analysis}. \todo{Add varied gamma BFs and recovered values.}}
  \begin{tabular}{ldd|d@{}dd}
  \hline \hline
   & \multicolumn{1}{c}{$A_\mathrm{common}$} & \multicolumn{1}{c}{Bayes Factor} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Bayes Factor} \\
  ephemeris & \multicolumn{1}{c}{[$\gamma_\mathrm{common}=13/3$]} & \multicolumn{1}{c}{2A--1} & \multicolumn{1}{c}{$A_\mathrm{common}$} & \multicolumn{1}{c}{$\gamma_\mathrm{common}$} & \multicolumn{1}{c}{2A--1}  \\
  \hline
  DE438 		& 1.96e-15 	& 35,092. & - & - & - \\
  INPOP19a 	& 1.92e-15	& 15,874. & - & - & - \\
  \hline
  \bayesephem & 1.56e-15	& 504. & - & - & - \\
  \hline
  \end{tabular}
  \end{center}
  \label{tab:crn_bfs}
\end{table*}

==> table_spatialcorrs_bfs_multCP.tex <==
% !TEX root = nanograv_12p5yr_gwb.tex

\begin{table*}
 \begin{center}
 \caption{Bayes factors for model comparison performed to examine the evidence for multiple common processes with different ORFs to be present in the data set. All models contain a common process with H.-D. correlations. The base model contains a single H.-D. correlated process, while the other models contain additional common process alongside an H.-D. correlated process. The digit in the parentheses gives the uncertainty on the last quoted digit.}
%
  	\begin{tabular}{ld@{}dd@{}dd@{}d}
		\hline\hline
		& \multicolumn{2}{c}{3B--3A: H.-D.+dipole corr. red process}
		& \multicolumn{2}{c}{3D--3A: H.-D.+monopole corr. red process} 
		& \multicolumn{2}{c}{3E--3A: H.-D.+uncorr. red process} \\
JPL ephemeris		& \multicolumn{6}{c}{vs.\ H.-D. correlated red process} \\
        & \multicolumn{1}{c}{$\gamma=13/3$} & \multicolumn{1}{c}{$\gamma \in [0,7]$}
        & \multicolumn{1}{c}{$\gamma=13/3$} & \multicolumn{1}{c}{$\gamma \in [0,7]$}
        & \multicolumn{1}{c}{$\gamma=13/3$} & \multicolumn{1}{c}{$\gamma \in [0,7]$} \\
    		\hline
            DE438           & 0.77(3) & 0.520(8) & 1.34(5) & 1.75(3) & 1.026(7) & 0.60(1) \\
        \hline
        \textsc{BayesEphem} & 0.63(2) & 0.500(7) & 1.65(5)  & 0.74(1) & 1.25(1) & 0.73(1) \\
    		\hline
	\end{tabular}
%	
	 \end{center}
 \label{tab:spatial_bfs_mult}
\end{table*}
